Dynamic Principal Projection for Cost-Sensitive Online Multi-Label Classification

We study multi-label classification (MLC) with three important real-world issues: online updating, label space dimensional reduction (LSDR), and cost-sensitivity. Current MLC algorithms have not been designed to address these three issues simultaneously. In this paper, we propose a novel algorithm, cost-sensitive dynamic principal projection (CS-DPP) that resolves all three issues. The foundation of CS-DPP is an online LSDR framework derived from a leading LSDR algorithm. In particular, CS-DPP is equipped with an efficient online dimension reducer motivated by matrix stochastic gradient, and establishes its theoretical backbone when coupled with a carefully-designed online regression learner. In addition, CS-DPP embeds the cost information into label weights to achieve cost-sensitivity along with theoretical guarantees. Experimental results verify that CS-DPP achieves better practical performance than current MLC algorithms across different evaluation criteria, and demonstrate the importance of resolving the three issues simultaneously.

==> 5_3.tex <==
\begin{figure}[t]
\begin{minipage}{.5\textwidth}
\centering
    \begin{subfigure}[b]{.5\textwidth}
                \includegraphics[width=\textwidth]{fig_new/yeast_ideal_comp_hamming_loss.png}
                %\caption{mediamill F1, $M$=$25\%K$}
                \caption{yeast Hamm}
                \label{fig:5-3:yeast-h}
        \end{subfigure}%
    \begin{subfigure}[b]{.5\textwidth}
                \includegraphics[width=\textwidth]{fig_new/CAL500_ideal_comp_hamming_loss.png}
                %\caption{yeast F1, $M$=$25\%K$}
                \caption{CAL500 Hamm}
                \label{fig:5-3:CAL500-h}
        \end{subfigure}%
    \caption{DPP vs O-PLST, $M = 10\%$ of $K$}
    \label{fig:5-3}
    \vspace{-1.5em}
\end{minipage}
\end{figure}


==> table_csdpp_other_25.tex <==
\resizebox{0.75\textwidth}{!}{
\begin{tabular}{cccccc }\hline
$\mathsf{Dataset}$ & $\mathsf{Alg.}$ & $\mathsf{Hamm. \, loss}$ & $\mathsf{F1 \, loss}$ & $\mathsf{Acc. \, loss}$ & $\mathsf{Norm. \, rank \, loss}$ \\ \hline
\multirow{4}{*}{$\mathsf{CAL500}$} & O-CS & ${0.8221 \pm 0.0018}$ & ${0.739 \pm 0.000}$ & $\mathbf{0.025 \pm 0.002}$ & ${0.849 \pm 0.000}$ \\ 
 & O-RAND & ${0.3374 \pm 0.0057}$ & ${0.734 \pm 0.006}$ & ${0.393 \pm 0.006}$ & ${0.843 \pm 0.004}$ \\ 
 & DPP & $\mathbf{0.1479 \pm 0.0002}$ & ${0.653 \pm 0.001}$ & ${0.397 \pm 0.001}$ & ${0.784 \pm 0.001}$ \\ 
 & CS-DPP & $\mathbf{0.1476 \pm 0.0001}$ & $\mathbf{0.602 \pm 0.001}$ & ${0.150 \pm 0.002}$ & $\mathbf{0.751 \pm 0.001}$ \\ \hline
\multirow{4}{*}{$\mathsf{Corel5k}$} & O-CS & ${0.9853 \pm 0.0002}$ & ${0.981 \pm 0.000}$ & $\mathbf{0.003 \pm 0.001}$ & ${0.991 \pm 0.000}$ \\ 
 & O-RAND & ${0.2857 \pm 0.0042}$ & ${0.978 \pm 0.001}$ & ${0.424 \pm 0.008}$ & ${0.989 \pm 0.000}$ \\ 
 & DPP & $\mathbf{0.0101 \pm 0.0000}$ & ${0.912 \pm 0.001}$ & ${0.467 \pm 0.000}$ & ${0.939 \pm 0.000}$ \\ 
 & CS-DPP & $\mathbf{0.0101 \pm 0.0000}$ & $\mathbf{0.844 \pm 0.000}$ & ${0.220 \pm 0.001}$ & $\mathbf{0.904 \pm 0.000}$ \\ \hline
\multirow{4}{*}{$\mathsf{emotions}$} & O-CS & ${0.5810 \pm 0.0085}$ & ${0.535 \pm 0.006}$ & ${0.174 \pm 0.023}$ & ${0.682 \pm 0.006}$ \\ 
 & O-RAND & ${0.3586 \pm 0.0096}$ & ${0.591 \pm 0.029}$ & ${0.319 \pm 0.023}$ & ${0.654 \pm 0.013}$ \\ 
 & DPP & $\mathbf{0.2807 \pm 0.0038}$ & ${0.446 \pm 0.011}$ & ${0.235 \pm 0.009}$ & ${0.531 \pm 0.005}$ \\ 
 & CS-DPP & $\mathbf{0.2819 \pm 0.0036}$ & $\mathbf{0.398 \pm 0.004}$ & $\mathbf{0.046 \pm 0.015}$ & $\mathbf{0.509 \pm 0.003}$ \\ \hline
\multirow{4}{*}{$\mathsf{enron}$} & O-CS & ${0.8025 \pm 0.0023}$ & ${0.878 \pm 0.001}$ & $\mathbf{0.106 \pm 0.008}$ & ${0.934 \pm 0.000}$ \\ 
 & O-RAND & ${0.3150 \pm 0.0109}$ & ${0.830 \pm 0.007}$ & ${0.329 \pm 0.020}$ & ${0.912 \pm 0.005}$ \\ 
 & DPP & $\mathbf{0.0599 \pm 0.0001}$ & ${0.528 \pm 0.002}$ & ${0.282 \pm 0.001}$ & $\mathbf{0.634 \pm 0.002}$ \\ 
 & CS-DPP & $\mathbf{0.0601 \pm 0.0002}$ & $\mathbf{0.519 \pm 0.001}$ & ${0.135 \pm 0.001}$ & $\mathbf{0.633 \pm 0.001}$ \\ \hline
\multirow{4}{*}{$\mathsf{mediamill}$} & O-CS & ${0.8832 \pm 0.0020}$ & ${0.915 \pm 0.000}$ & ${0.092 \pm 0.007}$ & ${0.956 \pm 0.000}$ \\ 
 & O-RAND & ${0.2854 \pm 0.0076}$ & ${0.879 \pm 0.007}$ & ${0.371 \pm 0.023}$ & ${0.940 \pm 0.003}$ \\ 
 & DPP & $\mathbf{0.0307 \pm 0.0000}$ & ${0.472 \pm 0.000}$ & ${0.306 \pm 0.000}$ & ${0.592 \pm 0.000}$ \\ 
 & CS-DPP & $\mathbf{0.0307 \pm 0.0000}$ & $\mathbf{0.457 \pm 0.000}$ & $\mathbf{0.068 \pm 0.000}$ & $\mathbf{0.580 \pm 0.000}$ \\ \hline
\multirow{4}{*}{$\mathsf{medical}$} & O-CS & ${0.8173 \pm 0.0018}$ & ${0.943 \pm 0.001}$ & ${0.090 \pm 0.005}$ & ${0.970 \pm 0.000}$ \\ 
 & O-RAND & ${0.2921 \pm 0.0134}$ & ${0.894 \pm 0.006}$ & ${0.261 \pm 0.023}$ & ${0.952 \pm 0.003}$ \\ 
 & DPP & $\mathbf{0.0150 \pm 0.0001}$ & ${0.377 \pm 0.004}$ & ${0.184 \pm 0.003}$ & ${0.402 \pm 0.005}$ \\ 
 & CS-DPP & $\mathbf{0.0152 \pm 0.0001}$ & $\mathbf{0.316 \pm 0.004}$ & $\mathbf{0.036 \pm 0.002}$ & $\mathbf{0.360 \pm 0.004}$ \\ \hline
\multirow{4}{*}{$\mathsf{nuswide}$} & O-CS & ${0.8721 \pm 0.0031}$ & ${0.957 \pm 0.000}$ & $\mathbf{0.319 \pm 0.010}$ & ${0.978 \pm 0.000}$ \\ 
 & O-RAND & ${0.2843 \pm 0.0119}$ & ${0.951 \pm 0.003}$ & ${0.593 \pm 0.014}$ & ${0.968 \pm 0.002}$ \\ 
 & DPP & $\mathbf{0.0201 \pm 0.0000}$ & ${0.672 \pm 0.000}$ & ${0.580 \pm 0.000}$ & ${0.690 \pm 0.000}$ \\ 
 & CS-DPP & $\mathbf{0.0201 \pm 0.0000}$ & $\mathbf{0.648 \pm 0.000}$ & $\mathbf{0.329 \pm 0.001}$ & $\mathbf{0.675 \pm 0.000}$ \\ \hline
\multirow{4}{*}{$\mathsf{scene}$} & O-CS & ${0.6286 \pm 0.0076}$ & ${0.676 \pm 0.004}$ & $\mathbf{0.155 \pm 0.017}$ & ${0.803 \pm 0.002}$ \\ 
 & O-RAND & ${0.2985 \pm 0.0205}$ & ${0.709 \pm 0.025}$ & ${0.304 \pm 0.028}$ & ${0.746 \pm 0.008}$ \\ 
 & DPP & $\mathbf{0.1788 \pm 0.0016}$ & ${0.911 \pm 0.005}$ & ${0.470 \pm 0.002}$ & ${0.927 \pm 0.003}$ \\ 
 & CS-DPP & $\mathbf{0.1797 \pm 0.0014}$ & $\mathbf{0.631 \pm 0.004}$ & $\mathbf{0.142 \pm 0.011}$ & $\mathbf{0.697 \pm 0.004}$ \\ \hline
\multirow{4}{*}{$\mathsf{yeast}$} & O-CS & ${0.5961 \pm 0.0060}$ & ${0.564 \pm 0.006}$ & ${0.205 \pm 0.018}$ & ${0.702 \pm 0.003}$ \\ 
 & O-RAND & ${0.3464 \pm 0.0111}$ & ${0.583 \pm 0.012}$ & ${0.356 \pm 0.021}$ & ${0.696 \pm 0.005}$ \\ 
 & DPP & $\mathbf{0.2136 \pm 0.0004}$ & ${0.423 \pm 0.002}$ & ${0.301 \pm 0.002}$ & ${0.539 \pm 0.003}$ \\ 
 & CS-DPP & $\mathbf{0.2144 \pm 0.0005}$ & $\mathbf{0.385 \pm 0.001}$ & $\mathbf{0.016 \pm 0.001}$ & $\mathbf{0.497 \pm 0.001}$ \\ \hline
\end{tabular}}


==> table_csdpp_other_50.tex <==
\resizebox{0.75\textwidth}{!}{
\begin{tabular}{cccccc }\hline
$\mathsf{Dataset}$ & $\mathsf{Alg.}$ & $\mathsf{Hamm. \, loss}$ & $\mathsf{F1 \, loss}$ & $\mathsf{Acc. \, loss}$ & $\mathsf{Norm. \, rank \, loss}$ \\ \hline
\multirow{4}{*}{$\mathsf{CAL500}$} & O-CS & ${0.8315 \pm 0.0011}$ & ${0.740 \pm 0.000}$ & $\mathbf{0.014 \pm 0.001}$ & ${0.849 \pm 0.000}$ \\ 
 & O-RAND & ${0.2620 \pm 0.0045}$ & ${0.703 \pm 0.006}$ & ${0.389 \pm 0.006}$ & ${0.824 \pm 0.004}$ \\ 
 & DPP & $\mathbf{0.1487 \pm 0.0002}$ & ${0.654 \pm 0.001}$ & ${0.396 \pm 0.001}$ & ${0.785 \pm 0.001}$ \\ 
 & CS-DPP & $\mathbf{0.1490 \pm 0.0002}$ & $\mathbf{0.602 \pm 0.001}$ & ${0.151 \pm 0.001}$ & $\mathbf{0.751 \pm 0.001}$ \\ \hline
\multirow{4}{*}{$\mathsf{Corel5k}$} & O-CS & ${0.9860 \pm 0.0002}$ & ${0.981 \pm 0.000}$ & $\mathbf{0.004 \pm 0.001}$ & ${0.991 \pm 0.000}$ \\ 
 & O-RAND & ${0.1687 \pm 0.0033}$ & ${0.971 \pm 0.002}$ & ${0.447 \pm 0.009}$ & ${0.986 \pm 0.001}$ \\ 
 & DPP & $\mathbf{0.0101 \pm 0.0000}$ & ${0.911 \pm 0.001}$ & ${0.467 \pm 0.000}$ & ${0.939 \pm 0.000}$ \\ 
 & CS-DPP & $\mathbf{0.0101 \pm 0.0000}$ & $\mathbf{0.842 \pm 0.001}$ & ${0.213 \pm 0.000}$ & $\mathbf{0.903 \pm 0.001}$ \\ \hline
\multirow{4}{*}{$\mathsf{emotions}$} & O-CS & ${0.5079 \pm 0.0096}$ & ${0.538 \pm 0.007}$ & ${0.225 \pm 0.014}$ & ${0.671 \pm 0.007}$ \\ 
 & O-RAND & ${0.3357 \pm 0.0086}$ & ${0.545 \pm 0.020}$ & ${0.360 \pm 0.015}$ & ${0.679 \pm 0.021}$ \\ 
 & DPP & $\mathbf{0.2276 \pm 0.0010}$ & ${0.470 \pm 0.007}$ & ${0.277 \pm 0.004}$ & ${0.546 \pm 0.005}$ \\ 
 & CS-DPP & $\mathbf{0.2306 \pm 0.0012}$ & $\mathbf{0.377 \pm 0.002}$ & $\mathbf{0.033 \pm 0.003}$ & $\mathbf{0.481 \pm 0.002}$ \\ \hline
\multirow{4}{*}{$\mathsf{enron}$} & O-CS & ${0.7172 \pm 0.0041}$ & ${0.872 \pm 0.001}$ & $\mathbf{0.138 \pm 0.009}$ & ${0.930 \pm 0.000}$ \\ 
 & O-RAND & ${0.2205 \pm 0.0079}$ & ${0.779 \pm 0.009}$ & ${0.314 \pm 0.009}$ & ${0.879 \pm 0.005}$ \\ 
 & DPP & $\mathbf{0.0642 \pm 0.0002}$ & ${0.527 \pm 0.001}$ & ${0.274 \pm 0.001}$ & $\mathbf{0.632 \pm 0.001}$ \\ 
 & CS-DPP & $\mathbf{0.0643 \pm 0.0001}$ & $\mathbf{0.522 \pm 0.001}$ & $\mathbf{0.129 \pm 0.001}$ & ${0.636 \pm 0.001}$ \\ \hline
\multirow{4}{*}{$\mathsf{mediamill}$} & O-CS & ${0.8998 \pm 0.0049}$ & ${0.916 \pm 0.001}$ & $\mathbf{0.060 \pm 0.003}$ & ${0.955 \pm 0.000}$ \\ 
 & O-RAND & ${0.1775 \pm 0.0107}$ & ${0.825 \pm 0.014}$ & ${0.331 \pm 0.015}$ & ${0.900 \pm 0.007}$ \\ 
 & DPP & $\mathbf{0.0307 \pm 0.0000}$ & ${0.472 \pm 0.000}$ & ${0.306 \pm 0.000}$ & ${0.592 \pm 0.000}$ \\ 
 & CS-DPP & $\mathbf{0.0307 \pm 0.0000}$ & $\mathbf{0.457 \pm 0.000}$ & $\mathbf{0.059 \pm 0.000}$ & $\mathbf{0.581 \pm 0.000}$ \\ \hline
\multirow{4}{*}{$\mathsf{medical}$} & O-CS & ${0.6863 \pm 0.0047}$ & ${0.937 \pm 0.001}$ & ${0.111 \pm 0.010}$ & ${0.966 \pm 0.000}$ \\ 
 & O-RAND & ${0.1673 \pm 0.0116}$ & ${0.836 \pm 0.012}$ & ${0.256 \pm 0.019}$ & ${0.911 \pm 0.005}$ \\ 
 & DPP & $\mathbf{0.0132 \pm 0.0001}$ & ${0.280 \pm 0.003}$ & ${0.136 \pm 0.001}$ & ${0.312 \pm 0.002}$ \\ 
 & CS-DPP & $\mathbf{0.0130 \pm 0.0001}$ & $\mathbf{0.250 \pm 0.002}$ & $\mathbf{0.019 \pm 0.001}$ & $\mathbf{0.299 \pm 0.002}$ \\ \hline
\multirow{4}{*}{$\mathsf{nuswide}$} & O-CS & ${0.8200 \pm 0.0053}$ & ${0.957 \pm 0.000}$ & ${0.321 \pm 0.008}$ & ${0.977 \pm 0.000}$ \\ 
 & O-RAND & ${0.1767 \pm 0.0097}$ & ${0.942 \pm 0.005}$ & ${0.556 \pm 0.011}$ & ${0.957 \pm 0.002}$ \\ 
 & DPP & $\mathbf{0.0201 \pm 0.0000}$ & ${0.672 \pm 0.000}$ & ${0.580 \pm 0.000}$ & ${0.690 \pm 0.000}$ \\ 
 & CS-DPP & $\mathbf{0.0201 \pm 0.0000}$ & $\mathbf{0.648 \pm 0.000}$ & $\mathbf{0.304 \pm 0.000}$ & $\mathbf{0.675 \pm 0.000}$ \\ \hline
\multirow{4}{*}{$\mathsf{scene}$} & O-CS & ${0.5023 \pm 0.0184}$ & ${0.664 \pm 0.008}$ & ${0.191 \pm 0.021}$ & ${0.771 \pm 0.005}$ \\ 
 & O-RAND & ${0.2678 \pm 0.0116}$ & ${0.633 \pm 0.017}$ & ${0.299 \pm 0.020}$ & ${0.699 \pm 0.018}$ \\ 
 & DPP & $\mathbf{0.1711 \pm 0.0020}$ & ${0.809 \pm 0.008}$ & ${0.423 \pm 0.003}$ & ${0.827 \pm 0.009}$ \\ 
 & CS-DPP & $\mathbf{0.1720 \pm 0.0015}$ & $\mathbf{0.558 \pm 0.003}$ & $\mathbf{0.104 \pm 0.009}$ & $\mathbf{0.623 \pm 0.004}$ \\ \hline
\multirow{4}{*}{$\mathsf{yeast}$} & O-CS & ${0.4504 \pm 0.0104}$ & ${0.524 \pm 0.009}$ & ${0.238 \pm 0.012}$ & ${0.666 \pm 0.008}$ \\ 
 & O-RAND & ${0.2926 \pm 0.0060}$ & ${0.500 \pm 0.013}$ & ${0.343 \pm 0.012}$ & ${0.649 \pm 0.013}$ \\ 
 & DPP & $\mathbf{0.2080 \pm 0.0003}$ & ${0.406 \pm 0.001}$ & ${0.291 \pm 0.001}$ & ${0.520 \pm 0.001}$ \\ 
 & CS-DPP & $\mathbf{0.2079 \pm 0.0003}$ & $\mathbf{0.382 \pm 0.001}$ & $\mathbf{0.026 \pm 0.001}$ & $\mathbf{0.492 \pm 0.001}$ \\ \hline
\end{tabular}}

